Account Verification on Social Media: User Perceptions and Paid Enrollment

We investigate how users perceive social media account verification, how those perceptions compare to platform practices, and what happens when a gap emerges. We use recent changes in Twitter's verification process as a natural experiment, where the meaning and types of verification indicators rapidly and significantly shift. The project consists of two components: a user survey and a measurement of verified Twitter accounts. In the survey study, we ask a demographically representative sample of U.S. respondents (n = 299) about social media account verification requirements both in general and for particular platforms. We also ask about experiences with online information sources and digital literacy. More than half of respondents misunderstand Twitter's criteria for blue check account verification, and over 80% of respondents misunderstand Twitter's new gold and gray check verification indicators. Our analysis of survey responses suggests that people who are older or have lower digital literacy may be modestly more likely to misunderstand Twitter verification. In the measurement study, we randomly sample 15 million English language tweets from October 2022. We obtain account verification status for the associated accounts in November 2022, just before Twitter's verification changes, and we collect verification status again in January 2022. The resulting longitudinal dataset of 2.85 million accounts enables us to characterize the accounts that gained and lost verification following Twitter's changes. We find that accounts posting conservative political content, exhibiting positive views about Elon Musk, and promoting cryptocurrencies disproportionately obtain blue check verification after Twitter's changes. We close by offering recommendations for improving account verification indicators and processes.

==> survey.tex <==
\small

Thank you for joining this study. Please answer the following questions based on your experiences with social media. Please \textbf{do not consult any external sources} when answering the questions.

\noindent [Question and response ordering may be altered or randomized.]

\begin{enumerate}
    \item During a typical week, how often do you \textbf{watch, read, or listen to news} from the following sources?

    (None / One day / Two days / Three days / Four days
/ Five days / Six days / Every day)

    \begin{itemize}
        \item TV
        \item Newspapers or print magazines
        \item  Radio
        \item  Online-only news websites
        \item Social media
        \item  Personal conversations
    \end{itemize}
    
    \item During a typical week, how often do you \textbf{see a post or video} from the following social media platforms?

    (None / One day / Two days / Three days / Four days
/ Five days / Six days / Every day)

    \begin{itemize}
        \item Facebook
        \item Instagram
        \item Snapchat
        \item TikTok
        \item Twitter
    \end{itemize}
    
    \item During a typical week, how often do you \textbf{use a personal account} with the following social media platforms?

        (None / One day / Two days / Three days / Four days
/ Five days / Six days / Every day)

    \begin{itemize}
        \item Facebook
        \item Instagram
        \item Snapchat
        \item TikTok
        \item Twitter
    \end{itemize}
    
    \item In general, what kinds of accounts do you follow on social media? Please select \textbf{all} that apply or select none of the above.

    \begin{enumerate}[label=(\alph*)]
        \item Celebrities and influencers
        \item Politicians, government officials, and government agencies
        \item Journalists and news outlets
        \item Friends and family
        \item Businesses and other organizations
        \item None of the above
    \end{enumerate}
    
    \item In general, when deciding whether to follow an account on social media, how important are the following factors? Please \textbf{rank} the following factors in order of importance, where 1 is the most important and 10 is the least important.

    \begin{enumerate}[label=(\alph*)]
        \item The account belongs to a person you know
        \item The account belongs to a notable person or organization
        \item The account has a “verified” badge
        \item The account has many followers
        \item The account frequently posts content
        \item The account posts content that interests you
        \item The account posts content that you agree with
        \item The account posts content that your followers agree with
        \item The account has been active on the platform for a long time
        \item The account follows you
    \end{enumerate}
    
    \item In general, when deciding whether to like, share, retweet, or otherwise interact with a post on social media, how important are the following factors? Please \textbf{rank} the following factors in order of importance, where 1 is the most important and 10 is the least important.

    \begin{enumerate}[label=(\alph*)]
        \item The post is from a person you know
        \item The post is from a notable person or organization
        \item The post is from an account with a “verified” badge
        \item The post is from an account with many followers
        \item The post is from an account that frequently posts content
        \item The post interests you
        \item The post expresses views that you agree with
        \item The post expresses views that your followers agree with
        \item The post is from an account that has been active on the platform for a long time
        \item The post is from an account that follows you
    \end{enumerate}
    
    \item Some accounts on social media platforms are “verified.” In general, what does a “verified” badge on an account \textbf{mean to you}?
    
    [Short free response.]
    
    \item In general, what steps \textbf{should be required} to verify an account on a social media platform?
    
    [Free response.]

    \item In general, what requirements \textbf{must} an account satisfy to become “verified” and obtain a “verified” badge on a social media platform? Please select \textbf{all} that apply or select none of the above.

    \begin{enumerate}[label=(\alph*)]
        \item The platform confirms the identity of the person or organization operating the account
        \item The platform confirms that the account is not impersonating a notable person or organization
        \item The platform calls or texts a telephone number associated with the account, and the platform confirms that the call or text was received
        \item The account frequently posts content on the platform
        \item The account belongs to a notable person or organization
        \item The account has many followers on the platform
        \item The account has been active on the platform for a long time
        \item The account has a paid subscription to the platform
        \item None of the above
    \end{enumerate}

    \item In general, what is \textbf{typically true} of an account with a “verified” badge on a social media platform? Please select \textbf{all} that apply or select none of the above.

    \begin{enumerate}[label=(\alph*)]
        \item The platform confirms the identity of the person or organization operating the account
        \item The platform confirms that the account is not impersonating a notable person or organization
        \item The platform calls or texts a telephone number associated with the account, and the platform confirms that the call or text was received
        \item The account frequently posts content on the platform
        \item The account belongs to a notable person or organization
        \item The account has many followers on the platform
        \item The account has been active on the platform for a long time
        \item The account has a paid subscription to the platform
        \item None of the above
    \end{enumerate}

    Some Twitter accounts, such as the account below, have a blue “verified” badge:
    \includegraphics[scale=0.02]{images/check_tw_blue.png} 

    \item Under Twitter’s current policies, what requirements \textbf{must} an account satisfy to become “verified” and obtain a blue “verified” badge? Please select \textbf{all} that apply or select none of the above.

    \begin{enumerate}[label=(\alph*)]
        \item Twitter confirms the identity of the person or organization operating the account
        \item Twitter confirms that the account is not impersonating a notable person or organization
        \item Twitter calls or texts a telephone number associated with the account, and Twitter confirms that the call or text was received
        \item The account frequently posts content on Twitter
        \item The account belongs to a notable person or organization
        \item The account has many followers on Twitter
        \item The account has been active on Twitter for a long time
        \item The account has a paid subscription to Twitter
        \item None of the above
    \end{enumerate}

    \item What is \textbf{typically true} of an account with a blue “verified” badge on Twitter? Please select \textbf{all} that apply or select none of the above.

    \begin{enumerate}[label=(\alph*)]
        \item Twitter confirms the identity of the person or organization operating the account
        \item Twitter confirms that the account is not impersonating a notable person or organization
        \item Twitter calls or texts a telephone number associated with the account, and Twitter confirms that the call or text was received
        \item The account frequently posts content on Twitter
        \item The account belongs to a notable person or organization
        \item The account has many followers on Twitter
        \item The account has been active on Twitter for a long time
        \item The account has a paid subscription to the Twitter
        \item None of the above
    \end{enumerate}

    [Repeat the above two questions with analogous phrasing and official accounts for a subset of Facebook, Instagram, TikTok, and YouTube.]

    \item In your experience, are there important differences between the “verified” badges on popular social media platforms? If you do not know, please respond “Do Not Know.”

    [Free response.]

    \item Some Twitter accounts have a gold “verified” badge: \includegraphics[scale=0.15]{images/check_tw_gold.png} 

    What does the gold color of the badge mean? If you do not know, please respond “Do Not Know.”

    [Free response.]

    \item Some Twitter accounts have a gray “verified” badge: 
    \includegraphics[scale=0.15]{images/check_tw_grey.png} 

    What does the gray color of the badge mean? If you do not know, please respond “Do Not Know.”

    [Free response.]

    \item Who is the current President of the United States?

    \begin{enumerate}[label=(\alph*)]
        \item Donald Trump
        \item Barack Obama
        \item George W. Bush
        \item Joe Biden
        \item Bill Clinton
    \end{enumerate}

    \item Who is the current leader of Twitter? If you do not know, please respond “Do Not Know.”

    [Free response.]

    \item People often read online news from a variety of sources, including TV channels, newspapers, and online-only outlets. Many of these sources are active on social media. Which of the following news sources do you read most often? Please ignore the prior question and select The Wall Street Journal and Axios.

    \begin{enumerate}[label=(\alph*)]
        \item The New York Times
        \item The Wall Street Journal
        \item MSNBC
        \item Fox News
        \item Axios
        \item Politico
        \item None of the above
    \end{enumerate}

    \item Have you ever had a personal or organizational account verified on a social media platform? Please select \textbf{all} that apply or select never verified.

    \begin{enumerate}[label=(\alph*)]
        \item Facebook
        \item Instagram
        \item Snapchat
        \item TikTok
        \item Twitter
        \item Other [Free response.]
        \item Never verified
    \end{enumerate}

    \item (If any for the prior question:) When verifying a personal or organizational social media account, what steps were you required to take?

    [Free response.]

    \item Have you ever provided your telephone number to a social media platform, then received a call or text from the platform to confirm that you have access to that number? 

        Yes
        
        No

    \item Suppose that a social media platform has the following requirements for an account to obtain a “verified” badge.
    \begin{itemize}
        \item The platform confirms that the account is not impersonating a notable person or organization
        \item The platform calls or texts a telephone number associated with the account, and the platform confirms that the call or text was received
        \item The account was created on the platform at least 90 days ago
        \item The account has a paid subscription to the platform
    \end{itemize}

    The platform does \textbf{not} confirm the identity of the person or organization operating the account. The account also need not belong to a notable person or organization, have many followers, or frequently post content on the platform.

    \begin{enumerate}[label=(\alph*)]
        \item Very sufficient
        \item Somewhat sufficient
        \item Neither sufficient nor insufficient
        \item Somewhat insufficient
        \item Very insufficient
    \end{enumerate}

    Would you consider the platform’s requirements for verifying accounts to be sufficient or insufficient?
    \item (If insufficient:) Why would you consider the platform's requirements for verifying accounts to be insufficient?

    [Free response]

    \item How familiar are you with the following computer and Internet-related items? 

    (No understanding / Little understanding / Some understanding / Good understanding /Full understanding)

    \begin{itemize}
        \item Hashtag
        \item Proxypod
        \item Tagging
        \item Status Update
        \item Advanced Search
        \item Preference Setting
        \item Tablet
        \item Malware
        \item App
        \item Selfie
    \end{itemize}

    \item (In pilot rounds:) Are there any questions in this survey that you found difficult to understand or to respond to?

    [Free response]

    \item (In pilot rounds:) Is there any feedback that you would like to provide about this survey?

    [Free response]

\end{enumerate}
